High-resolution synthetic residential energy use profiles for the United States

Efficient energy consumption is crucial for achieving sustainable energy goals in the era of climate change and grid modernization. Thus, it is vital to understand how energy is consumed at finer resolutions such as household in order to plan demand-response events or analyze the impacts of weather, electricity prices, electric vehicles, solar, and occupancy schedules on energy consumption. However, availability and access to detailed energy-use data, which would enable detailed studies, has been rare. In this paper, we release a unique, large-scale, synthetic, residential energy-use dataset for the residential sector across the contiguous United States covering millions of households. The data comprise of hourly energy use profiles for synthetic households, disaggregated into Thermostatically Controlled Loads (TCL) and appliance use. The underlying framework is constructed using a bottom-up approach. Diverse open-source surveys and first principles models are used for end-use modeling. Extensive validation of the synthetic dataset has been conducted through comparisons with reported energy-use data. We present a detailed, open, high-resolution, residential energy-use dataset for the United States.

==> vv_cluster.tex <==
\subsection*{II. Comparing energy use patterns (load shape/structural similarity)}

\begin{figure*}[!h]    
    \begin{subfigure}{.495\textwidth}
    \centering
    \includegraphics[width=8.25cm,height=11cm]{experiment2_distances.png}
    \caption{Case 1: $closeness(\mathscr{R},\mathscr{S})$}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.25cm,height=11cm]{experiment4_distances.png}
    \caption{Case 2: $closeness(\mathscr{S},\mathscr{R})$}
      \label{fig:}
    \end{subfigure}
    
    \caption{\textbf{Example of \emph{closeness} in different cases with varying $k$.} Figures show the distances of data points from sets  $\mathscr{R}$ and $\mathscr{S}$ to their respective cluster center. (a) demonstrates histograms of distances for different $k$. The plot on left is for real data points and on right is for synthetic data points. Then, we calculate $closeness(\mathscr{R},\mathscr{S})$ using Hellinger distance (corresponds blue line in Figure~\ref{fig:overall-vv-results}(c)). For $k=5$ a bimodal pattern is observed in distances for synthetic data points which tends to diminish as the number of clusters $k$ increases.  Figure (b) shows histograms of distances for different $k$ for case 2. The plot on left is for synthetic data points and on right is for real data points.  $closeness(\mathscr{S},\mathscr{R})$ is calculated using Hellinger distance (corresponds to orange line in Figure~\ref{fig:overall-vv-results}(c)).
    }
    \label{fig:closeness_proximity}
\end{figure*}


\begin{figure*}[!h]    
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=7.5cm,height=5.5cm]{coverage_plot_exp_2_4.png}
    \caption{Coverage}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=7.5cm,height=5.5cm]{closeness_plot_exp_2_4.png}
    \caption{Closeness}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{Summary of the two case scenarios.} Orange color is denoted for findings of case 1 where we cluster real data set $\mathscr{R}$ and assign a cluster label to synthetic data set $\mathscr{S}$. Blue color is denoted for findings of case 1 where we cluster synthetic data set $\mathscr{S}$ and assign a cluster label to real data set $\mathscr{R}$. (a) illustrates 100\% coverage in both cases even as $k$ varies. This means that, in each case at least one data point belongs to every cluster for a given $k$. (b) shows the closeness between the two distance vectors : distance of real data points in a cluster to its respective centroid and  distance of synthetic data points in a cluster to its respective centroid. Closeness is given by the Hellinger distance which suggests that a value of 0 signifies that the two distributions are similar. The value of distances is close to 0 for all values of $k$ in both the cases. However, an upward trend is observed as $k$ increases. Overall we see the robustness of results w.r.t. $k$.} 
    \label{fig:overall-vv-results}
\end{figure*}


In this section, the synthetic energy use timeseries are evaluated using the concepts of diversity, coverage, and closeness. 
The diversity in energy use patterns is captured by segmenting the normalized timeseries $\langle \overline{e}_0,\ldots,\overline{e}_{23}\rangle$  using unsupervised learning techniques such as clustering.
This is followed by studying \emph{coverage} in terms of what percentage of synthetic timeseries population is represented in the real timeseries population and vice versa. Thus, coverage is used to measure  diversity.
However, learning only coverage is not sufficient. It is necessary to measure the accuracy of the matches found. Hence, we introduce the \emph{closeness} metric. It studies how close (e.g. $dist(i,j)$) are the synthetic and real data points.

Let $\mathscr{R}$ and $\mathscr{S}$ be the set of load shapes of real and synthetic energy use timeseries. 
Let $K_\mathscr{R}$ be the number of unique load shapes (segments/patterns/clusters) found in set $\mathscr{R}$.
Then, we define the ${coverage(\mathscr{S})}$ as a ratio

\begin{equation}
\begin{array}{l}
    coverage(\mathscr{S})\;=\;\frac{\textrm{Number of unique shapes in $\mathscr{R}$ that contain atleast one data point from $\mathscr{S}$}}{\textrm{Number of unique shapes in $\mathscr{R}$}} \\ \\
   \quad \quad \quad \quad \quad \; \; =\;\frac{1}{K_\mathscr{R}} \times \sum_{b=1}^{K_\mathscr{R}} \mathbb{I}_b
    \quad \text{where}   \\ \\
    \mathbb{I}_b\;=\; \begin{cases}
      1 & \text{if cluster $b$ contains atleast one timeseries $j\in\mathscr{S}$ }\;,\\
      0 & \text{otherwise.}
    \end{cases}    
    \end{array}
\end{equation}

\noindent
Thus, $coverage(\mathscr{S})$ reflects the degree to which samples from set $\mathscr{S}$ cover the patterns in set $\mathscr{R}$.
Similarly, if $K_\mathscr{S}$ is the number of unique segments in set $\mathscr{S}$, then,  $coverage(\mathscr{R})$ reflects the the percentage of unique patterns in set $\mathscr{S}$ covered by data points in set $\mathscr{R}$.
Coverage is bounded between 0 and 1.
Figure~\ref{fig:} shows $coverage(\mathscr{S})$ and $coverage(\mathscr{R})$ as $K$ varies.


To measure closeness we calculate distance of individual timeseries to it's respective cluster center/representative.
If $K_\mathscr{R}$ is the number of clusters in set $\mathscr{R}$, then, the \emph{closeness($\mathscr{S}$,$\mathscr{R}$)} of set $\mathscr{S}$ to set $\mathscr{R}$ is measured by comparing the distributions of distances of individual timeseries $i\in\mathscr{R}$ and $j\in\mathscr{S}$ in each cluster $c\in K_\mathscr{R}$ to the respective center/representative timeseries of the cluster.
Figure~\ref{fig:} illustrates the schematic of building the distance distributions.
Let $P_\mathscr{R}$ and $P_\mathscr{S}$ denote the probability vectors of distances of sets $\mathscr{R}$ and $\mathscr{S}$ respectively. To measure the degree of closeness, we compare the two probability distributions using Hellinger distance $\mathsf{H}(P_\mathscr{R},P_\mathscr{S})$ (Equation~\ref{eq:hellinger}).
If distributions $P_\mathscr{R}$ and $P_\mathscr{R}$ are similar, then we say that set $\mathscr{S}$ is close to set $\mathscr{R}$.
\begin{equation}
   closeness(\mathscr{S},\mathscr{R}) \;=\; \mathsf{H}(P_\mathscr{R},P_\mathscr{S})
\end{equation}
Closeness is bounded between 0 and 1. 0 implies that the two sets are close. 
Note that closeness is not a symmetric metric i.e. 
$closeness(\mathscr{S},\mathscr{R}) \neq closeness(\mathscr{R},\mathscr{S})$.
Figure~\ref{fig:} describes the variation in similarity score of the probability with different number of segments $K$.

Now, we briefly describe the experimental setup. Two cases are considered to examine coverage, closeness and robustness of cluster groupings ($k$). 
For each case the energy use timeseries is normalized resulting in a \emph{load shape} $\langle \overline{e}_0,\ldots,\overline{e}_{23}\rangle$.
We choose normalization by total consumption~(Equation~\ref{eq:total-normalization}) in order to consider pronounced effects of peak-load in the profile.
Household preferences or lifestyles can be typically captured by one or more load shapes~\cite{kwac2014}, hence we choose this representation for uncovering patterns in the data. 
Thus, every $i \in \mathscr{R}$ and $j \in \mathscr{S}$ are normalized energy use vectors of length 24.

\begin{equation}\label{eq:total-normalization}
    \overline{e}_t\;=\;\frac{e_t}{E^\mathsf{total}}\;,\quad \textrm{where} \; \; E^\mathsf{total} = \sum^{23}_{t=0} e_t
\end{equation}












In the first case (Case 1), we generate $K_\mathscr{R}$ patterns from set $\mathscr{R}$ by clustering the real normalized energy use vectors using k-means clustering algorithm with Euclidean distance.
This is followed by assigning a cluster label $k\in K_\mathscr{R}$ to each synthetic energy use timeseries $j\in \mathscr{S}$. Let $c_k$ be the center/representation vector of group $k$.
Then, $j \in \mathscr{S}$ is assigned to the cluster whose cluster center distance is minimum from $j$ and is given by 
%$min_{\forall k \in K_\mathscr{R}}  dist(j,c_k)$.
$min(dist(j,c_0),\ldots, dist(j,c_{K_\mathscr{R}}))$.
Then, we calculate the coverage of synthetic data $coverage(\mathscr{S})$ and closeness of synthetic data to real data among all clusters as $closeness(\mathscr{S},\mathscr{R})$.
In Case 2, we generate $K_\mathscr{S}$ clusters from set $\mathscr{S}$ (synthetic data) by segmenting the normalized energy use vectors using k-means clustering algorithm with Euclidean distance.
This is followed by assigning a cluster label $k\in K_\mathscr{S}$ to each real energy use timeseries $i\in \mathscr{R}$. $i$ is assigned to the cluster whose cluster center distance is minimum from $i$ and is given by $min_{\forall k \in K_\mathscr{S}}  dist(i,c_k)$.
Then, we calculate the coverage of real data in synthetic groups $coverage(\mathscr{R})$ and closeness of real data and synthetic data among all synthetic clusters as $closeness(\mathscr{R},\mathscr{S})$.


Results of both the cases are summarized in Figures~\ref{fig:overall-vv-results}.
A 100\% \emph{coverage} is observed in both the cases for different values of $k$.
Observations for \emph{closeness} metric are interesting. The Hellinger distance is close to zero in all the scenarios, however there is a slight uptake in the value as $k$ increases. 
We inspect this further in Figure~\ref{fig:closeness_proximity}.
Figure~\ref{fig:closeness_proximity} shows histograms of distances of real data points and synthetic data points from their assigned cluster center.
In case 1, the distribution of distances of synthetic data points is slightly broader than the distribution of distances of real data points for all $k$. Thus, we see a distance for \emph{closeness($\mathscr{R},\mathscr{S}$)} in Figure~\ref{fig:overall-vv-results}(c).
As $k$ increases it is observed that some individual clusters have a broad and/or bimodal distance distribution indicating that there are data points that are very close to the cluster center while a few are far away. This difference is apparent as the number of clusters increases. 


The goal of this V\&V exercise was to verify if the diversity and trends of the real energy use profiles are replicated in the synthetic energy use profiles.
Due to a biased and skewed sample of the real energy use data, it is challenging to perform validation of synthetic data.
Some of the characteristics of the real datasets that hinder the  implementation of using existing evaluation metrics \emph{as is} are mentioned below.
No supporting information of the real households is available (e.g. household size, dwelling type, square footage, indoor thermostat setting).
We have shown that all of these factors are extremely important in the generation of household demand at a given time.
Some of households in the real data may also be participants in demand-response programs resulting in unique load shapes due to shifting demand/reducing peak demand that may not be found in households not participating in DR programs (e.g. synthetic data).
The real datasets are collected for different years for each region.
The data are incomplete for some regions (e.g. San Diego samples do not have lighting data).
The sample size (number of households) is highly skewed. It varies from 9 households in Montana to 56000 households for Horry,SC.
Thus, it is important to note that $|\mathscr{R}|<<|\mathscr{S}|$ (e.g. the number of households simulated in our framework for Washington state is far greater than that of 78 households in real data for Washington state.) 
All of these observations are summarized in Table~\ref{tab:validation-datasets}.







==> vv_regional.tex <==
\subsection*{III. Observing differences and similarities in synthetic energy use data in spatially representative locations}


\begin{figure*}[!h]    
    \begin{subfigure}{.17\textwidth}
    \centering
    \includegraphics[width=3cm,height=3cm]{Arlington_pie.png}
    \caption{Arlington, VA}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.17\textwidth}
    \centering
    \includegraphics[width=3cm,height=3cm]{Cook_pie.png}
    \caption{Cook, IL}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.17\textwidth}
    \centering
    \includegraphics[width=3cm,height=3cm]{Houston_pie.png}
    \caption{Houston, TX}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.17\textwidth}
    \centering
    \includegraphics[width=3cm,height=3cm]{Maricopa_pie.png}
    \caption{Maricopa, AZ}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.17\textwidth}
    \centering
    \includegraphics[width=3cm,height=3cm]{King_pie.png}
    \caption{King, WA}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.13\textwidth}
    \centering
    \includegraphics[width=2cm,height=2.9cm]{pie_legend.png}
    \caption{Legend}
      \label{fig:}
    \end{subfigure}
    
    \caption{\textbf{Composition of synthetic electric consumption in the representative target locations.} Heating and cooling constitute the majority part of the residential electric consumption. Refrigerators consume slightly higher energy in hotter regions such as Maricopa and Houston. Activities such as dishwashing, laundry, and cooking represents between 8-17\% for different regions. Lighting and water heating have a consistent proportion of consumption across all locations. The proportions bear similarities with data published by EIA.}
    \label{fig:pie-chart-regional}
\end{figure*}

% overview of the study and selected locations
This empirical study uses only the synthetic data to conduct a comparative regional analyses to examine similarities and dissimilarities between energy use for different end-uses.
We observe the spatio-temporal patterns and variations in different end-uses with respect to environmental elements such as irradiance and temperature as well as demographic and structural characteristics of the households.
The selected target locations are spatially representative of different climate zones of the U.S.:

\begin{center}
\emph{Arlington, VA}; \emph{Cook County, IL}; \emph{Houston County, TX}; \emph{Maricopa County, AZ}; \emph{King County, WA} \end{center}



% composition of energy consumption
The composition of electric consumption by end-uses is shown in the form of pie diagrams in Figure~\ref{fig:pie-chart-regional}.
EIA reports the shares of the major end-uses as follows: DHW 17-32\%, lighting 5-10\%, refrigerator 3-5\%, activities/appliances 20-26\%, space heating 25-47\%, and air conditioning 5-10\%.
In general, the percentages of major end-use categories lie in the ranges similar to those reported by EIA.
HVAC has a dominant share in the energy consumption in households as compared to usage of appliances and/or other activities.

\begin{figure*}[!h]    
    \begin{subfigure}{.24\textwidth}
    \centering
    \includegraphics[width=4.2cm,height=2.8cm]{hvac_daily_timeseries-variation.png}
    \caption{HVAC energy use}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \centering
    \includegraphics[width=4.2cm,height=2.8cm]{refr_daily_timeseries-variation.png}
    \caption{Refrigerator energy use}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \centering
    \includegraphics[width=4.2cm,height=2.8cm]{h2o_daily_timeseries-variation.png}
    \caption{Hot water energy use}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
    \centering
    \includegraphics[width=4.2cm,height=2.8cm]{F_timeseries.png}
    \caption{Outside temperature}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{Monthly synthetic energy use changes in end-uses such as HVAC, refrigerator, domestic hot water w.r.t. temperature.} The above line charts monthly energy use changes in end-uses such as HVAC, refrigerator, domestic hot water w.r.t. outside temperature.
    The line chart shows average daily consumption over all households in the target regions. The scatter plot in the background describes average daily consumption for an end-use for sampled days color coded by location. The size of the markers denotes the standard deviation of the end-use consumption. Legend: Arlington, VA (green); Cook County, IL (blue); Houston County, TX (yellow); Maricopa County, AZ (brown); King County, WA (cyan) }
    \label{fig:regional-linechart-major}
\end{figure*}


\begin{figure*}[!h]    
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=2.5cm]{dwasher_daily_timeseries-variation.png}
    \caption{Dishwasher}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=2.5cm]{laundry_daily_timeseries-variation.png}
    \caption{Laundry}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=2.5cm]{cook_daily_timeseries-variation.png}
    \caption{Cook}
      \label{fig:}
    \end{subfigure}
    
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=2.5cm]{cleaning_daily_timeseries-variation.png}
    \caption{Cleaning}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=2.5cm]{tv_daily_timeseries-variation.png}
    \caption{TV use}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=5.5cm,height=3cm]{computer_daily_timeseries-variation.png}
    \caption{Computer use}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{Synthetic appliance energy use variation in target locations throughout the year.} The line charts show variation in daily energy consumption for different appliance energy use throughout the year averaged by month. The lines depict average daily consumption over all households in the target region. The scatter plot in the background describes average daily consumption for an end-use for sampled days color coded by location. The size of the markers denotes the standard deviation of the end-use consumption. There are noticeable similarities in appliance-usage throughout all locations indicating that people in different parts of the country use appliances in a similar style. This is a reasonable observation since day-to-day activities such as cooking and cleaning will occur in all households. Their usage pattern may change during the day, but the total energy consumed by the appliance at the end of the day is similar. Arlington, VA (green); Cook County, IL (blue); Houston County, TX (yellow); Maricopa County, AZ (brown); King County, WA (cyan)}
    \label{fig:regional-linechart-activities}
\end{figure*}

Seasonal energy use variations for HVAC, refrigerator, and hot water is captured in Figure~\ref{fig:regional-linechart-major}.
The plot shows variation in daily average energy use of the four end-uses on a monthly basis alongwith temperature across the year 2014.
Refrigerator energy use increases slightly with temperature while energy used to heat water decreases with increase in temperature. 


% hot water
Electricity usage for heating water is the lowest during summer months for all locations (Figure~\ref{fig:regional-linechart-major}c). 
In particular, regions from hot-humid and hot-dry climate zones consume the least amount of energy.
This observation stems from the relation between $E^{\mathsf{h2o,v}}$ and $T^{\mathsf{cold}}_{m,z}$ described in Equation~\ref{eq:dhw}.
The water inlet temperature ( $T^{\mathsf{cold}}_{m,z}$) differs across temporal as well as spatial scale and is dependent on outside environment temperatures~\cite{NRELhotwater129} (Details in Appendix). 
Figure~\ref{fig:regional-h2o-charts} shows plots describing relation between household size and the number of gallons of hot water consumed and energy required to heat water.
Note that, we consider only electric water heaters in this work.


%hvac
Figure~\ref{fig:regional-linechart-major}(a) shows that the HVAC consumption varies significantly throughout the year. HVAC use is higher in hot-dry areas in summer as compared to other regions possibly due to higher temperatures. 
Structural characteristics such as dwelling size (square footage), insulation quality, age and efficiency of HVAC equipment also affect household HVAC consumption. 
Another important variable that drives HVAC consumption is indoor thermostat behavior which is related to household occupants' behavior/actions. In this work, indoor thermostat temperatures are set constant throughout the day. 
Insulation quality is not monitored in households (due to lack of data). We assume that the dwelling is well-insulated and the insulation values are implemented according to the DOE standards for the respective climate zones. 
In Figure~\ref{fig:hvac-sqft-light-hhsize}a we show effect of square footage (conditioned space) of a dwelling on hvac energy use.
In general, we observe that as the conditioned space in the dwelling increases, the HVAC consumption increases. 

%lighting
Lighting energy-use varies by seasons in all regions as irradiance levels change with weather events and seasons.
Figure~\ref{fig:regional-lighting-heatmap}b shows average irradiance time series for the target locations. The corresponding lighting usage is shown in Figure~\ref{fig:regional-lighting-heatmap}a.
As an example, we look at monthly irrandiance profiles across 24 hours in Virginia for the year 2014~(Figure~\ref{fig:regional-lighting-heatmap}d). The corresponding monthly lighting energy use time series is shown in Figure~\ref{fig:regional-lighting-heatmap}c.
Example of lighting consumption w.r.t. household size is explored in Figure~\ref{fig:hvac-sqft-light-hhsize}b.

Figure~\ref{fig:regional-linechart-activities} shows the breakdown of appliance usage for different appliances and electronic devices.
Both figures show a line chart indicating average daily consumption for the month. 
The scatter plot in the background describes average daily consumption for an end-use for sampled days color coded by location, where 
the size of the markers denotes the standard deviation of the end-use consumption.
It is observed that appliance usage in activities such as cooking, dishwashing, performing laundry, watching TV, using computer, and cleaning are fairly similar in different regions.
The above comment is intuitively true since appliance use duration and their ratings may not vary across regions.
However, the occurrence timing throughout the day may vary from house to house depending upon occupant schedules irrespective of which geographic regions they belong to.









\begin{figure*}[!h]    
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=4cm]{hvac_sqft_m2_winter.png}
    \caption{HVAC vs. house area (i.e. floor area)}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=4cm]{light_hhsize_winter.png}
    \caption{Lighting vs. household size}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{(a) Synthetic HVAC use and house area (i.e. floor area).} Boxplot comparing daily HVAC consumption in a winter day for the selected target locations by house area (i.e. floor area). The x-axis groups floor area of houses in five bins denoted in two units sq. ft ($\text{ft}^2$)  and sq m ($\text{m}^2$). The bins are as follows : $\leq$ 1000 $\text{ft}^2$, 1000 - 1500 $\text{ft}^2$, 1500 - 2000 $\text{ft}^2$, 2000 - 3000 $\text{ft}^2$, $\geq$ 3000 $\text{ft}^2$. It is observed that as floor area of the house increases HVAC consumption increases in all regions. Winter temperatures are relatively moderate in AZ and TX, thus, the HVAC consumption is less as compared to other regions. \textbf{(b) Synthetic lighting use and household size.} Lighting consumption increases as household size increases. Household size indicates number of members in a household.
    }
    \label{fig:hvac-sqft-light-hhsize}
\end{figure*}

\begin{figure*}[!h]    
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=3.8cm]{h2o_dailyGallonsHotH2o_winter.png}
    \caption{Hot water (gallons) vs. household size}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=3.8cm]{h2o_hhsize_winter.png}
    \caption{Hot water (energy) vs. household size}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{Synthetic hot water usage and energy vs. synthetic household size.} Household size indicates number of household members. The clustered bar charts show the amount of hot water consumed (in gallons in (a)) and corresponding energy usage in (b) according to household size in a winter day. The vertical black line on each bar shows the variation. Water usage and its variation increases with household size. The amount of energy for hot water end-use increases with household size and differs by region.} 
    \label{fig:regional-h2o-charts}
\end{figure*}

\begin{figure*}[!h]    
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.6cm,height=3.7cm]{light_heatmap_locations.png}
    \caption{Lighting profile}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.6cm,height=3.7cm]{irradiance_heatmap_locations.png}
    \caption{Irradiance profile}
    \end{subfigure}
    
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=4.8cm]{light_heatmap_VA.png}
    \caption{VA lighting profile}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=8.5cm,height=4.8cm]{irradiance_heatmap_VA.png}
    \caption{VA irradiance profile}
    \end{subfigure}
    
    \caption{\textbf{Heatmap depicting relation between hourly synthetic lighting usage and hourly irradiance.}  (a) shows average annual 24-hour lighting profiles of representative target locations. (b) shows average annual 24-hour irradiance profile of representative target locations. (c) and (d) present the variation in lighting usage and corresponding irradiance profiles at monthly level for Arlington, VA. (c) presents lighting consumption variation throughout the day in different months across the year. (d) shows variation in monthly irradiance profile. The units of measurements for energy usage is kWh and irradiance is Watts/m$^2$.  The lighting energy use is inversely proportional to the irradiance. The energy usage is higher in evening and night hours when the occupant is active in the dwelling. The average lighting and irradiance profiles show regional differences in irradiance availability and subsequent lighting energy usage. The VA profiles show that the day light is available for longer durations leading to lower lighting energy consumption as compared to winter.  }
    \label{fig:regional-lighting-heatmap}
\end{figure*}












==> vv_stat.tex <==
\subsection*{I. Comparing real and synthetic end-use energy usage (magnitude)}


\begin{figure*}[!h]    
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{hvac_jensenshannon_heatmap-short.png}
    \caption{HVAC (Jensen-Shannon)}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{hvac_hellinger_heatmap-short.png}
    \caption{HVAC  (Hellinger)}
      \label{fig:}
    \end{subfigure}
    
    
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{refr_jensenshannon_heatmap-short.png}
    \caption{Refrigerator  (Jensen-Shannon)}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{refr_hellinger_heatmap-short.png}
    \caption{Refrigerator (Hellinger)}
      \label{fig:}
    \end{subfigure}
    
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{cook_jensenshannon_heatmap-short.png}
    \caption{Cooking appliances  (Jensen-Shannon)}
      \label{fig:}
    \end{subfigure}
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=6.6cm,height=6.1cm]{cook_hellinger_heatmap-short.png}
    \caption{Cooking appliances (Hellinger)}
      \label{fig:}
    \end{subfigure}
    \caption{\textbf{Left column: Jensen-Shannon distance matrices, Right column: Hellinger distance matrices}. Each of the column shows Jensen-Shannon distance and Hellinger distance matrices between end-use probability distributions. Each matrix represents distances between two energy usage distributions for a particular enduse (e.g. HVAC, refrigerator, cooking). The row and column headers of the matrix represent different data-sources and different regions and each cell represents the probability distribution similarity/distance value in the form of heatmap, where the bar shows the range of the values on a continuous scale. }
    \label{fig:jensen-hellinger}
\end{figure*}


In this experiment, distributions of synthetic and real daily end-use data are compared using statistical metrics.
One way of comparing these distributions is by measuring distance between the real and synthetic end-use distributions.
Many metrics can be used to perform this task (e.g., Kullback–Leibler divergence (KL), the Hellinger distance, total variation distance (TVD), the Wasserstein metric, the Jensen-Shannon divergence (JS), and the Kolmogorov–Smirnov statistic (KS)).
Klemenjak et al.~\cite{Klemenjak2020} use JS distance and Hellinger distance as examples to compare distributions of appliance energy use between different datasets.
A similar method is implemented in this section using the JS distance and the Hellinger distance metric.
In our case, computing the distances between daily end use distributions allows us to perform regional comparisons as well as comparisons between real and synthetic datasets.

The Jensen-Shannon distance is the square root of the Jensen-Shannon divergence~\cite{JS1991}. The range of this metric ranges between $[0,1]$ where~0 implies the distributions are similar. 
We prefer JS divergence over KL divergence since it is a symmetric measure.
If~$P$ and~$Q$ are two probability vectors, then the JS distance~$\mathsf{JS}(P,Q)$ is given by 
\begin{equation}
    \mathsf{JS}(P,Q)\;=\;\sqrt{\frac{\mathsf{KL}(P||M)+\mathsf{KL}(Q||M)}{2}} \;,
\end{equation}
\noindent
where~$M$ is the pointwise mean of~$P$ and~$Q$ and~$\mathsf{KL}$  is the Kullback-Leibler divergence.
To supplement our study, we use Hellinger distance as a second metric to quantify the similarity between two probability distributions.
Hellinger distance is also a symmetric measure. Its range of values is $[0,1]$ with~0 encoding that the distributions are similar.
The Hellinger distance of two probability vectors~$P$ and~$Q$ is denoted by~$\mathsf{H}(P,Q)$ and defined as
\begin{equation}\label{eq:hellinger}
    \mathsf{H}(P,Q)\;=\;\frac{1}{\sqrt{2}}\sqrt{\sum^{k}_{i=1} (\sqrt{p_i} - \sqrt{q_i})^{2}} \;,
\end{equation}
\noindent
where~$k$ is the length of the vectors, and~$p_i$,~$q_i$ are the~$i^{\text{th}}$ elements of the vectors~$P$ and~$Q$, respectively.

Daily end-use energy usage (e.g. ${E}^{\mathsf{hvac}}_i$) at household level are compared in the real and synthetic data for every location specified in Table~\ref{tab:validation-datasets}.
Vectors $P$ and $Q$ denote values in a single end-use for two datasets.
Tables~\ref{fig:jensen-hellinger}(a)(b)(c) list JS distances and Tables~\ref{fig:jensen-hellinger}(d)(e)(f) list Hellinger distances for selected end-uses (HVAC, refrigerator, cooking appliances). 
Each matrix represents distances between two energy usage distributions for an end-use.
The row and column headers represent different data-sources and different regions and each cell represents the probability distribution similarity/distance value in the form of heatmap where the bar shows the range of the values on a continuous scale. 

The JS and Hellinger distance tables for end-uses show strong similarities (the distance is close to zero).
Furthermore, within each matrix three types of comparisons are performed. We compute similarity between end-use distributions for different regions within synthetic data, different regions within real data, and different regions in different data sources (namely real and synthetic data).
For appliance usage (e.g. cooking), the distributions are quite  similar across regions and data-sources.
This supports findings from Figure~\ref{fig:regional-linechart-activities} that there exists significant similarities between different regions for synthetic daily energy consumption of different appliances. 
For HVAC end-use, it is observed that the distributions grow apart between regions for both -- synthetic and real data sources. This is particularly true due to the strong association of HVAC with outdoor/environment temperature conditions and the time span for which these temperature conditions prevail (e.g., warmer temperatures are observed for a longer time in Texas (TX))





